BlockHouse: Blockchain-based Distributed Storehouse System

We propose in this paper BlockHouse, a decentralized/P2P storage system fully based on private blockchains. Each participant can rent his unused storage in order to host data of other members. This system uses a dual Smart Contract and Proof of Retrievability system to automatically check at a fixed frequency if the file is still hosted. In addition to transparency, the blockchain allows a better integration with all payments associated to this type of system ( regular payments, sequestration to ensure good behaviors of users, ...). Except the data transferred between the client and the server, all the actions go through a smart contract in the blockchain in order to log, pay and secure the entire storage process.

==> Makefile <==
#-----------------------------------------------------------------------------
# Basic parameters
#-----------------------------------------------------------------------------
# Softwares used. Please verify they are installed.
LATEX=pdflatex
LATEXMK=latexmk

# Target
ifeq ($(MAIN),)
MAIN=main
endif

#-----------------------------------------------------------------------------


#-----------------------------------------------------------------------------
# Advanced parameters
#-----------------------------------------------------------------------------
# LATEX options
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode

# LATEXMK options
LATEXMKOPT=-pdf
CONTINUOUS=-pvc

SOURCES= $(shell find *.tex)
FIGURES := $(shell find images/* -type f)

#-----------------------------------------------------------------------------

#-----------------------------------------------------------------------------
# Makefile body
#-----------------------------------------------------------------------------
all: $(MAIN).pdf

.refresh:
	touch .refresh

$(MAIN).pdf: .refresh $(SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
		-pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

force:
	touch .refresh
	rm $(MAIN).pdf
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
		-pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

clean:
	$(LATEXMK) -C $(MAIN)
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.aux *.end *.fls *.log *.out *.fdb_latexmk

once:
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

debug:
	$(LATEX) $(LATEXOPT) $(MAIN)

.PHONY: clean force once all

.PRECIOUS: $(MAIN).pdf

#-----------------------------------------------------------------------------

